Denjoy-Wolff points on the bidisk via models

Let $F=(\phi, \psi):\mathbb{D}^2\to\mathbb{D}^2$ denote a holomorphic self-map of the bidisk without interior fixed points. It is well-known that, unlike the case with self-maps of the disk, the sequence of iterates $$\{F^n:=F\circ F\circ \cdots \circ F\}$$ needn't converge. The cluster set of $\{F^n\}$ was described in a classical 1954 paper of Herv\'{e}. Motivated by Herv\'{e}'s work and the Hilbert space perspective of Agler, McCarthy and Young on boundary regularity, we propose a new approach to boundary points of Denjoy-Wolff type for the coordinate maps $\phi, \psi.$ We establish several equivalent descriptions of our Denjoy-Wolff points, some of which only involve checking specific directional derivatives and are particularly convenient for applications. Using these tools, we are able to refine Herv\'{e}'s theorem and show that, under the extra assumption of $\phi$ and $\psi$ possessing Denjoy-Wolff points with certain regularity properties, one can draw much stronger conclusions regarding the behavior of $\{F^n\}.$

==> Bibliography.tex <==
@article {AbateRaissynonsmoothconvex,
    AUTHOR = {Abate, Marco and Raissy, Jasmin},
     TITLE = {Wolff-{D}enjoy theorems in nonsmooth convex domains},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {193},
      YEAR = {2014},
    NUMBER = {5},
     PAGES = {1503--1518},
}
@article {ATYgeneralizedmodels,
    AUTHOR = {Agler, J. and Tully-Doyle, R. and Young, N. J.},
     TITLE = {Boundary behavior of analytic functions of two variables via
              generalized models},
   JOURNAL = {Indag. Math. (N.S.)},
  FJOURNAL = {Koninklijke Nederlandse Akademie van Wetenschappen.
              Indagationes Mathematicae. New Series},
    VOLUME = {23},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {995--1027},
}
@article {AMYfacial,
    AUTHOR = {Agler, Jim and McCarthy, John E. and Young, N. J.},
     TITLE = {Facial behaviour of analytic functions on the bidisc},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {43},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {478--494},
}
@article {AMYcaratheodory,
    AUTHOR = {Agler, Jim and McCarthy, John E. and Young, N. J.},
     TITLE = {A {C}arath\'{e}odory theorem for the bidisk via {H}ilbert space
              methods},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {352},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {581--624},
}
@article {BickelKneseassociated,
    AUTHOR = {Bickel, Kelly and Knese, Greg},
     TITLE = {Inner functions on the bidisk and associated {H}ilbert spaces},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {265},
      YEAR = {2013},
    NUMBER = {11},
     PAGES = {2753--2790},
}
@article {BickelKnesecanonicalAgler,
    AUTHOR = {Bickel, Kelly and Knese, Greg},
     TITLE = {Canonical {A}gler decompositions and transfer function
              realizations},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {368},
      YEAR = {2016},
    NUMBER = {9},
     PAGES = {6293--6324},
}
@article {BPSderivativesrationalinner,
    AUTHOR = {Bickel, Kelly and Pascoe, James Eldred and Sola, Alan},
     TITLE = {Derivatives of rational inner functions: geometry of
              singularities and integrability at the boundary},
   JOURNAL = {Proc. Lond. Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {116},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {281--329},
}
@article {BPSlevelcurveportraits,
    AUTHOR = {Bickel, Kelly and Pascoe, James Eldred and Sola, Alan},
     TITLE = {Level curve portraits of rational inner functions},
   JOURNAL = {Ann. Sc. Norm. Super. Pisa Cl. Sci. (5)},
  FJOURNAL = {Annali della Scuola Normale Superiore di Pisa. Classe di
              Scienze. Serie V},
    VOLUME = {21},
      YEAR = {2020},
     PAGES = {449--494},
}
@article {ChuLieBalls,
    AUTHOR = {Chu, Cho-Ho},
     TITLE = {Iteration of holomorphic maps on {L}ie balls},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {264},
      YEAR = {2014},
     PAGES = {114--154},
}
@article {ChuRigbyHilbertballs,
    AUTHOR = {Chu, Cho-Ho and Rigby, Michael},
     TITLE = {Iteration of self-maps on a product of {H}ilbert balls},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {411},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {773--786},
      ISSN = {0022-247X},
}
@article {ChuRigbyhoroballs,
    AUTHOR = {Chu, Cho-Ho and Rigby, Michael},
     TITLE = {Horoballs and iteration of holomorphic maps on bounded
              symmetric domains},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {311},
      YEAR = {2017},
     PAGES = {338--377},
}
@incollection {FrosiniDynamics,
    AUTHOR = {Frosini, Chiara},
     TITLE = {Dynamics on bounded domains},
 BOOKTITLE = {The {$p$}-harmonic equation and recent advances in analysis},
    SERIES = {Contemp. Math.},
    VOLUME = {370},
     PAGES = {99--117},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2005},
}
@article {FrosiniBusemann,
    AUTHOR = {Frosini, Chiara},
     TITLE = {Busemann functions and the {J}ulia-{W}olff-{C}arath\'{e}odory
              theorem for polydiscs},
   JOURNAL = {Adv. Geom.},
  FJOURNAL = {Advances in Geometry},
    VOLUME = {10},
      YEAR = {2010},
    NUMBER = {3},
     PAGES = {435--463},
}
@article {HERVE,
    AUTHOR = {Herv\'{e}, Michel},
     TITLE = {It\'{e}ration des transformations analytiques dans le
              bicercle-unit\'{e}},
   JOURNAL = {Ann. Sci. Ecole Norm. Sup. (3)},
  FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Troisi\`eme
              S\'{e}rie},
    VOLUME = {71},
      YEAR = {1954},
}
@article {McPascoerevisited,
    AUTHOR = {McCarthy, John E. and Pascoe, James E.},
     TITLE = {The {J}ulia-{C}arath\'{e}odory theorem on the bidisk revisited},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {83},
      YEAR = {2017},
    NUMBER = {1-2},
     PAGES = {165--175},
      ISSN = {0001-6969},
}
@article {McPascoencJulia,
    AUTHOR = {McCarthy, John E. and Pascoe, James E.},
     TITLE = {A non-commutative {J}ulia inequality},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {370},
      YEAR = {2018},
    NUMBER = {1-2},
     PAGES = {423--446},
      ISSN = {0025-5831},
}
@article {MellonDWboundesymmetric,
    AUTHOR = {Mellon, P.},
     TITLE = {Denjoy-{W}olff theory for finite-dimensional bounded symmetric
              domains},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {195},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {845--855},
      ISSN = {0373-3114},
}
@article {Mellonfiniterank,
    AUTHOR = {Mellon, P.},
     TITLE = {A {W}olff theorem for finite rank bounded symmetric domains},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {456},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {57--68},
      ISSN = {0022-247X},
}
@article {Pascoeinductive,
    AUTHOR = {Pascoe, J. E.},
     TITLE = {An inductive {J}ulia-{C}arath\'{e}odory theorem for {P}ick
              functions in two variables},
   JOURNAL = {Proc. Edinb. Math. Soc. (2)},
  FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {61},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {647--660},
      ISSN = {0013-0915},
}
@article {PSTcontrolledtangential,
    AUTHOR = {Pascoe, J. E. and Sargent, Meredith and Tully-Doyle, Ryan},
     TITLE = {A controlled tangential {J}ulia-{C}arath\'{e}odory theory via
              averaged {J}ulia quotients},
   JOURNAL = {Anal. PDE},
  FJOURNAL = {Analysis \& PDE},
    VOLUME = {14},
      YEAR = {2021},
    NUMBER = {6},
     PAGES = {1773--1795},
      ISSN = {2157-5045},
}
@article {SolaTullydynamics,
    AUTHOR = {Sola, Alan and Tully-Doyle, Ryan},
     TITLE = {Dynamics of low-degree rational inner skew-products on
              {$\Bbb{T}^2$}},
   JOURNAL = {Ann. Polon. Math.},
  FJOURNAL = {Annales Polonici Mathematici},
    VOLUME = {128},
      YEAR = {2022},
    NUMBER = {3},
     PAGES = {249--273},
      ISSN = {0066-2216},
}
@article {Tullyboundarysingularities,
    AUTHOR = {Tully-Doyle, Ryan},
     TITLE = {Analytic functions on the bidisk at boundary singularities via
              {H}ilbert space methods},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {11},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {55--70},
      ISSN = {1846-3886},
}
@book {Nowell,
    AUTHOR = {Nowell, Jason},
     TITLE = {Denjoy-Wolff sets for analytic maps on the polydisk},
      NOTE = {Thesis (Ph.D.)--University of Florida},
      YEAR = {2019},
}

@article {AbateJuliaWolff,
    AUTHOR = {Abate, Marco},
     TITLE = {The {J}ulia-{W}olff-{C}arath\'{e}odory theorem in polydisks},
   JOURNAL = {J. Anal. Math.},
  FJOURNAL = {Journal d'Analyse Math\'{e}matique},
    VOLUME = {74},
      YEAR = {1998},
     PAGES = {275--306},
      ISSN = {0021-7670},
}
@article {Valironabelpolydisc,
    AUTHOR = {Arosio, Leandro and Gumenyuk, Pavel},
     TITLE = {Valiron and {A}bel equations for holomorphic self-maps of the
              polydisc},
   JOURNAL = {Internat. J. Math.},
  FJOURNAL = {International Journal of Mathematics},
    VOLUME = {27},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {1650034, 16},
}
@article {Cartanbornes,
    AUTHOR = {Cartan, Henri},
     TITLE = {Sur les fonctions de {$n$} variables complexes: les
              transformations du produit topologique de deux domaines
              born\'{e}s},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'{e}t\'{e} Math\'{e}matique de France},
    VOLUME = {64},
      YEAR = {1936},
     PAGES = {37--48},
      ISSN = {0037-9484},
}
@article {Favre,
    AUTHOR = {Favre, Charles},
     TITLE = {Les applications monomiales en deux dimensions},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {51},
      YEAR = {2003},
    NUMBER = {3},
     PAGES = {467--475},
      ISSN = {0026-2285},
}
@article {PujalsShubdynamics,
    AUTHOR = {Pujals, Enrique R. and Shub, Michael},
     TITLE = {Dynamics of two-dimensional {B}laschke products},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {28},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {575--585},
}
@article {PujalsRoederergodic,
    AUTHOR = {Pujals, Enrique R. and Roeder, Roland K. W.},
     TITLE = {Two-dimensional {B}laschke products: degree growth and ergodic
              consequences},
   JOURNAL = {Indiana Univ. Math. J.},
  FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {59},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {301--325},
}
@article {Denjoy,
    AUTHOR = {Denjoy, A.},
     TITLE = {Sur l'it\'{e}ration des fonctions analytiques },
   JOURNAL = {C. R. Acad. Sc. Paris},
    VOLUME = {182},
      YEAR = {1926},
     PAGES = {255--257},
}
@article {Wolff1,
    AUTHOR = {Wolff, J.},
     TITLE = {Sur l'it\'{e}ration des fonctions born\'{e}es},
   JOURNAL = {C. R. Acad. Sc. Paris},
    VOLUME = {182},
      YEAR = {1926},
     PAGES = {200-201},
}
@article {Wolff2,
    AUTHOR = {Wolff, J.},
     TITLE = { Sur l'it\'{e}ration des fonctions holomorphes dans une r\'{e}gion, et dont les valeurs
appartiennent \`{a} cette r \'{e}gion},
   JOURNAL = {C. R. Acad. Sc. Paris},
    VOLUME = {182},
      YEAR = {1926},
     PAGES = {42-43},
}
@article {Wolff3,
    AUTHOR = {Wolff, J.},
     TITLE = {Sur une g\'{e}n\'{e}ralisation d'un th\'{e}or\`{e}me de Schwarz},
   JOURNAL = {C. R. Acad. Sc. Paris},
    VOLUME = {182},
      YEAR = {1926},
     PAGES = {918-920},
}
@article {Burckel,
    AUTHOR = {Burckel, R. B.},
     TITLE = {Iterating analytic self-maps of discs},
   JOURNAL = {Amer. Math. Monthly},
  FJOURNAL = {American Mathematical Monthly},
    VOLUME = {88},
      YEAR = {1981},
    NUMBER = {6},
     PAGES = {396--407},
}
@book {Abatebook,
    AUTHOR = {Abate, Marco},
     TITLE = {Iteration theory of holomorphic maps on taut manifolds},
    SERIES = {Research and Lecture Notes in Mathematics. Complex Analysis
              and Geometry},
 PUBLISHER = {Mediterranean Press, Rende},
      YEAR = {1989},
     PAGES = {xvii+417},
}
@article {Maccluer,
    AUTHOR = {MacCluer, Barbara D.},
     TITLE = {Iterates of holomorphic self-maps of the unit ball in {${\bf
              C}\sp{N}$}},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {30},
      YEAR = {1983},
    NUMBER = {1},
     PAGES = {97--106},
}
@article {Herveball,
    AUTHOR = {Herv\'{e}, Michel},
     TITLE = {Quelques propri\'{e}t\'{e}s des applications analytiques d'une boule \`a
              {$m$} dimensions dan elle-m\^{e}me},
   JOURNAL = {J. Math. Pures Appl. (9)},
  FJOURNAL = {Journal de Math\'{e}matiques Pures et Appliqu\'{e}es. Neuvi\`eme S\'{e}rie},
    VOLUME = {42},
      YEAR = {1963},
     PAGES = {117--147},
}
@article {Abatestronglyconvex,
    AUTHOR = {Abate, Marco},
     TITLE = {Horospheres and iterates of holomorphic maps},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {198},
      YEAR = {1988},
    NUMBER = {2},
     PAGES = {225--238},
      ISSN = {0025-5874},
}
@article {Abatecompactly,
    AUTHOR = {Abate, Marco},
     TITLE = {Iteration theory, compactly divergent sequences and commuting
              holomorphic maps},
   JOURNAL = {Ann. Scuola Norm. Sup. Pisa Cl. Sci. (4)},
  FJOURNAL = {Annali della Scuola Normale Superiore di Pisa. Classe di
              Scienze. Serie IV},
    VOLUME = {18},
      YEAR = {1991},
    NUMBER = {2},
     PAGES = {167--191},
      ISSN = {0391-173X},
}
@article {Huang,
    AUTHOR = {Huang, Xiao Jun},
     TITLE = {A non-degeneracy property of extremal mappings and iterates of
              holomorphic self-mappings},
   JOURNAL = {Ann. Scuola Norm. Sup. Pisa Cl. Sci. (4)},
  FJOURNAL = {Annali della Scuola Normale Superiore di Pisa. Classe di
              Scienze. Serie IV},
    VOLUME = {21},
      YEAR = {1994},
    NUMBER = {3},
     PAGES = {399--419},
}
@article {TranVu,
    AUTHOR = {Khanh, Tran Vu and Thu, Ninh Van},
     TITLE = {Iterates of holomorphic self-maps on pseudoconvex domains of
              finite and infinite type in {$\Bbb{C}^n$}},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {144},
      YEAR = {2016},
    NUMBER = {12},
     PAGES = {5197--5206},
}
@article {Zhang,
    AUTHOR = {Zhang, Wenjun and Ren, Fyuao},
     TITLE = {Dynamics on weakly pseudoconvex domains},
      NOTE = {A Chinese summary appears in Chinese Ann. Math. Ser. A
              {{\bf{1}}6} (1995), no. 6, 798},
   JOURNAL = {Chinese Ann. Math. Ser. B},
  FJOURNAL = {Chinese Annals of Mathematics. Series B},
    VOLUME = {16},
      YEAR = {1995},
    NUMBER = {4},
     PAGES = {467--476},
}
@article {BudCn,
    AUTHOR = {Budzy\'{n}ska, Monika},
     TITLE = {The {D}enjoy-{W}olff theorem in {$\Bbb C^n$}},
   JOURNAL = {Nonlinear Anal.},
  FJOURNAL = {Nonlinear Analysis. Theory, Methods \& Applications. An
              International Multidisciplinary Journal},
    VOLUME = {75},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {22--29},
}
@article {BudDWtype,
    AUTHOR = {Budzy\'{n}ska, Monika and Kuczumow, Tadeusz and Reich, Simeon},
     TITLE = {Theorems of {D}enjoy-{W}olff type},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {192},
      YEAR = {2013},
    NUMBER = {4},
     PAGES = {621--648},
}
@article {Budcondensing,
    AUTHOR = {Budzy\'{n}ska, Monika},
     TITLE = {The {D}enjoy-{W}olff theorem for condensing mappings in a
              bounded and strictly convex domain in a complex {B}anach
              space},
   JOURNAL = {Ann. Acad. Sci. Fenn. Math.},
  FJOURNAL = {Annales Academi\ae  Scientiarum Fennic\ae . Mathematica},
    VOLUME = {39},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {919--940}
     }
     @book {Sarason,
    AUTHOR = {Sarason, Donald},
     TITLE = {Sub-{H}ardy {H}ilbert spaces in the unit disk},
    SERIES = {University of Arkansas Lecture Notes in the Mathematical
              Sciences},
    VOLUME = {10},
      NOTE = {A Wiley-Interscience Publication},
 PUBLISHER = {John Wiley \& Sons, Inc., New York},
      YEAR = {1994},
     PAGES = {xvi+95},
}
@book {Caratheod,
    AUTHOR = {Caratheodory, C.},
     TITLE = {Theory of functions of a complex variable. {V}ol. 2},
      NOTE = {Translated by F. Steinhardt},
 PUBLISHER = {Chelsea Publishing Co., New York},
      YEAR = {1954},
     PAGES = {220},
}
@article {Julia,
    AUTHOR = {Julia, Gaston},
     TITLE = {Extension nouvelle d'un lemme de {S}chwarz},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {42},
      YEAR = {1920},
    NUMBER = {1},
     PAGES = {349--355},
}
@article {Wlod,
    AUTHOR = {W\l odarczyk, Kazimierz},
     TITLE = {Julia's lemma and {W}olff's theorem for {$J^\ast$}-algebras},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {99},
      YEAR = {1987},
    NUMBER = {3},
     PAGES = {472--476},
}
@book {OldPick,
    AUTHOR = {Agler, Jim and McCarthy, John E.},
     TITLE = {Pick interpolation and {H}ilbert function spaces},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {44},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2002},
     PAGES = {xx+308},
      ISBN = {0-8218-2898-3},
}
@book {NewPick,
    AUTHOR = {Agler, Jim and McCarthy, John Edward and Young, Nicholas},
     TITLE = {Operator analysis---{H}ilbert space methods in complex
              analysis},
    SERIES = {Cambridge Tracts in Mathematics},
    VOLUME = {219},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2020},
     PAGES = {xv+375},
      ISBN = {978-1-108-48544-9},
}
@misc{FrosiniArxiv,
  
  url = {https://arxiv.org/abs/math/0402014},
  
  author = {Frosini, Chiara},
  
  title = {Dynamics in the complex bidisc},
  
  publisher = {arXiv},
  
  year = {2004},
  
}
@inproceedings {EarleHam,
    AUTHOR = {Earle, Clifford J. and Hamilton, Richard S.},
     TITLE = {A fixed point theorem for holomorphic mappings},
 BOOKTITLE = {Global {A}nalysis ({P}roc. {S}ympos. {P}ure {M}ath., {V}ols.
              {XIV}, {XV}, {XVI}, {B}erkeley, {C}alif., 1968)},
     PAGES = {61--65},
 PUBLISHER = {Amer. Math. Soc., Providence, R.I.},
      YEAR = {1970},
}
